Characterization of the Imbalance Problem on Complete Bipartite Graphs

We study the imbalance problem on complete bipartite graphs. The imbalance problem is a graph layout problem and is known to be NP-complete. Graph layout problems find their applications in the optimization of networks for parallel computer architectures, VLSI circuit design, information retrieval, numerical analysis, computational biology, graph theory, scheduling and archaeology. In this paper, we give characterizations for the optimal solutions of the imbalance problem on complete bipartite graphs. Using the characterizations, we can solve the imbalance problem in $\mathcal{O}(\log(|V|) \cdot \log(\log(|V|)))$ time, when given the cardinalities of the parts of the graph, and verify whether a given solution is optimal in $O(|V|)$ time on complete bipartite graphs. We also introduce a restricted form of proper interval bipartite graphs on which the imbalance problem is solvable in $\mathcal{O}(c \cdot \log(|V|) \cdot \log(\log(|V|)))$ time, where $c = \mathcal{O}(|V|)$, by using the aforementioned characterizations.

==> sections/conclusion.tex <==
\section{Conclusion and future work}\label{c5}
We have shown that the imbalance problem is solvable in linear time on restricted PI-bigraphs, when given a corresponding family of maximal subsets. We believe that a similar proof structure can be applied to restricted PI-bigraphs with a relaxed restriction. Instead of limiting the number of overlapping vertices in consecutive vertex sets $C_i$ and $C_{i+1}$ to exactly 1, we limit it to at most 2 and at least 1. %That is, given the following definition:
%\begin{definition}
%	A PI-bigraph $G = (X,Y,E)$ is a relaxed restricted PI-bigraph, if there exists a family of maximal subsets $\mathscr{C}=\{C_1, \dots, C_n\}$ such that
%	$$\big(\forall_{1\leq i < n}~ 1 \leq |C_i \cap C_{i+1}| \leq 2\big) \wedge \big(\forall_{1\leq i < j < n}~j-i > 1 \implies C_i \cap C_j = \emptyset\big).$$
%\end{definition}
%We believe that a similar analysis can be applied to show the linear time solvability of relaxed restricted PI-bigraphs, when given a corresponding family of maximal subsets.

An interesting research direction would be to see whether it is possible to compute a family of maximal subsets $\mathscr{C}$ efficiently. Perhaps it is possible to compute $\mathscr{C}$ efficiently by using the ordering analogous to the proper interval ordering mentioned in the introduction.

%We hope that it is possible to show that the imbalance problem on restricted PI-bigraphs with an unbounded number of overlapping vertices in two consecutive vertex sets of $\mathscr{C}$ is linear time solvable. This will generalize our result to (unrestricted) PI-bigraphs. The interaction between the overlapping vertices within the intersection makes this case difficult to analyze.

==> sections/references.tex <==


%
% ---- Bibliography ----
%
% BibTeX users should specify bibliography style 'splncs04'.
% References will then be sorted and formatted in the correct style.
%
% \bibliographystyle{splncs04}
% \bibliography{mybibliography}
%
\begin{thebibliography}{8}
\bibitem{ref_article1}
Author, F.: Article title. Journal \textbf{2}(5), 99--110 (2016)

\bibitem{ref_lncs1}
Author, F., Author, S.: Title of a proceedings paper. In: Editor,
F., Editor, S. (eds.) CONFERENCE 2016, LNCS, vol. 9999, pp. 1--13.
Springer, Heidelberg (2016). \doi{10.10007/1234567890}

\bibitem{ref_book1}
Author, F., Author, S., Author, T.: Book title. 2nd edn. Publisher,
Location (1999)

\bibitem{ref_proc1}
Author, A.-B.: Contribution title. In: 9th International Proceedings
on Proceedings, pp. 1--2. Publisher, Location (2010)

\bibitem{ref_url1}
LNCS Homepage, \url{http://www.springer.com/lncs}. Last accessed 4
Oct 2017
\end{thebibliography}
